On the kappa ring of $\overline{M}_{g,n}$

Let $\kappa_e(\overline{M}_{g,n})$ denote the kappa ring of $\overline{M}_{g,n}$ in codimension $e$. For $g,e\geq 0$ fixed, as the number $n$ of the markings grows large we show that the rank of $\kappa_e(\overline{M}_{g,n})$ is asymptotic to $$\frac{{n+e\choose e}{g+e\choose e}}{(e+1)!}\simeq \frac{{g+e\choose e}n^e}{e!(e+1)!}.$$ When $g\leq 2$ we show that a kappa class $\kappa$ is trivial if and only if the integral of $\kappa$ against all boundary strata is trivial. For $g=1$ we further show that the rank of $\kappa_{n-d}(\overline{M}_{1,n})$ is equal to $|P_1(d,n-d)|$, where $P_i(d,k)$ denotes the set of partitions $p=(p_1,...,p_\ell)$ of $d$ such that at most $k$ of the numbers $p_1,...,p_\ell$ are greater than $i$.

==> standardcommand.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bigoplu}{\sum}
\newcommand{\Ps}{\psi}
\newcommand{\ovl}{\overline}
\newcommand{\ocal}{\mathfrak{o}}
\newcommand{\ofrak}{\mathfrak{o}}
\newcommand{\rrr}{{\mathfrak{r}}}
\newcommand{\Nbar}{\overline{\mathcal{N}}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\val}{\mathrm{val}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Image}{\mathrm{Im}}
\newcommand{\pp}{\mathrm{p}}
\newcommand{\ppp}{\mathfrak{p}}
\newcommand{\Pm}{\widehat{\PP}}
\newcommand{\Pp}{\mathbb{P}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\n}{\mathrm{\bf{n}}}
\newcommand{\nn}{\mathrm{\bf{n}}}
\newcommand{\mm}{\mathrm{\bf{m}}}
\newcommand{\qqq}{\mathfrak{q}}
\newtheorem{question}{Question}
\newcommand{\tP}{\widetilde{\mathrm{P}}}
\newcommand{\point}{\mathrm{pt}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\SCC}{stable weighted graph }
\newcommand{\Tors}{\mathrm{Tors}}
\newcommand{\rk}{\mathrm{rk}}
\newtheorem{theorem}{Theorem}
\newtheorem{thm}{Theorem}[section]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{claim}[thm]{Claim}
\newtheorem{example}[thm]{Example}
\newtheorem{defn}[thm]{Definition}
\newtheorem{addendum}[thm]{Addendum}
\newtheorem{remark}[thm]{Remark}
\newtheorem{constr}[thm]{Construction}
\newtheorem{quest}{Question}[section]

\def\proof{\vspace{2ex}\noindent{\bf Proof.} }
\def\endproof{\relax\ifmmode\expandafter\endproofmath\else
  \unskip\nobreak\hfil\penalty50\hskip.75em\hbox{}\nobreak\hfil\bull
  {\parfillskip=0pt \finalhyphendemerits=0 \bigbreak}\fi}
\def\endproofmath$${\eqno\bull$$\bigbreak}
\def\bull{\vbox{\hrule\hbox{\vrule\kern3pt\vbox{\kern6pt}\kern3pt\vrule}\hrule}}
\newcommand{\smargin}[1]{\marginpar{\tiny{#1}}}
%\newcommand{\smargin}[1]{}
\newcounter{bean}
\newcommand{\Aut}{\mathrm{Aut}}
\newcommand{\Rel}{\mathrm{Rel}}
\newcommand{\alphas}{{\mbox{\boldmath$\alpha$}}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\PP}{\mathrm{P}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Quat}{\mathbb{H}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\QQ}{\mathrm{Q}}
\newcommand{\sig}{\sigma}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\ov}{\widehat}
\newcommand{\Det}{\mathrm{Det}}
\newcommand{\rank}{\mathrm{rank}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Mbar}{\overline{\mathcal{M}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\z}{\mathrm{\bf{z}}}
\newcommand{\w}{\mathrm{\bf{w}}}
\newcommand{\p}{\mathrm{\bf{p}}}
\newcommand{\q}{\mathrm{\bf{q}}}
\newcommand{\rr}{\mathrm{\bf{r}}}
\newcommand{\la}{\mathrm{\bf{y}}}
\newcommand{\lo}{\mathrm{\bf{x}}}
\newcommand{\lam}{\lambda}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ka}{\kappa}
\newcommand{\kring}{\ka^*\left(\Modbar_{g,n}\right)}
\newcommand{\kringc}{\ka^*_c\left(\Modbar_{g,n}\right)}
\newcommand{\Mgnbar}{\Modbar_{g,n}}
\newcommand{\Mgn}{\Mod_{g,n}}
\newcommand{\PPhi}{\overline{\Phi}}
\newcommand{\PPsi}{\overline{\Psi}}
\newcommand{\UU}{\overline{\mathbb{U}}}
\newcommand{\Fb}{\mathbb{F}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\MM}{\overline{\mathbb{M}}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\CFKT}{\text{CFK}}
\newcommand{\HFKT}{\text{HFK}}
\newcommand{\CFT}{\mathrm{CF}}
\newcommand{\HFT}{\mathrm{HF}}
\newcommand{\CFKTT}{\text{\emph{CFK}}}
\newcommand{\HFKTT}{\text{\emph{HFK}}}
\newcommand{\AAA}{\overline{\mathbb{A}}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\EE}{{\mathbb{E}}}
\newcommand{\A}{\mathbb{A}}
\newcommand{\Ahat}{\widehat{\mathbb{A}}}
\newcommand{\Bhat}{\widehat{\mathbb{B}}}
\newcommand{\Dhat}{\widehat{\mathbb{D}}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\M}{\mathbb{M}}
%\newcommand{\T}{\mathbb{T}}
\newcommand{\m}{\mathfrak{m}}
\newcommand{\Domain}{\mathcal{D}}
\newcommand{\gbar}{\overline{g}}
%\newcommand{\hbar}{\overline{h}}
\newcommand{\fbar}{\overline{f}}
\newcommand{\xfrak}{\mathfrak{x}}
\newcommand{\yfrak}{\mathfrak{y}}
\newcommand{\Gi}{\mathcal{G}}
\newcommand{\ut}{\underline{t}}
\newcommand{\us}{\underline{s}}
\newcommand{\ui}{\underline{i}}
\newcommand{\PN}{{\mathbb{P}^N}}
%\newcommand{\Group}{\mathfrak{G}}
\newcommand{\GroupH}{\mathfrak{H}}
\newcommand{\al}{\alpha}
\newcommand{\bet}{\beta}
\newcommand{\ParMod}{\mathcal{P}}
\newcommand{\MapMod}{\mathcal{X}}
\newcommand{\Almost}{\mathcal{J}}
\newcommand{\Inv}{\mathcal{I}}
\newcommand{\lra}{\longrightarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\Sig}{\Sigma}
\newcommand{\jsig}{{j_\Sigma}}
\newcommand{\Mod}{\mathcal{M}}
\newcommand{\Modbar}{{\overline{\mathcal{M}}}}
\newcommand{\Ci}{{\mathcal{C}}}
\newcommand{\Cibar}{{\overline{\mathcal{C}}}}
\newcommand{\xra}{\xrightarrow}
\newcommand{\Space}{\mathcal{Y}}
\newcommand{\Bundle}{\mathcal{E}}
\newcommand{\Homi}{\text{Hom}^{0,1}}
\newcommand{\dbar}{\overline{\partial}}
\newcommand{\ModX}{\mathcal{M}_g(X,\beta)}
\newcommand{\ModGX}{\mathcal{M}^\Group_g(X,\beta)}
\newcommand{\ModGXpar}{\mathcal{M}^\Group_g(X,\beta;(J;v))}
\newcommand{\ModXpar}{\mathcal{M}_g(X,\beta;(J;v))}
\newcommand{\Orbit}{\mathcal{O}}
\newcommand{\Ker}{\mathrm{Ker}}
\newcommand{\Cok}{\mathrm{Coker}}
%\newcommand{\m}{\mathfrak{m}}
\newcommand{\Div}{\mathcal{D}}
\newcommand{\DivGm}{\mathcal{D}^\Group_\m}
\newcommand{\Divm}{\mathcal{D}_\m}
\newcommand{\DivG}{\mathcal{D}^\Group}
\newcommand{\e}{\epsilon}
\newcommand{\thet}{{\overline{\theta}}}
\newcommand{\muu}{{\overline{\mu}}}
\newcommand{\zet}{{\overline{\zeta}}}
\newcommand{\et}{{\overline{\eta}}}
\newcommand{\PathMod}{\mathcal{Q}(\gamma_0,\gamma_1)}
\newcommand{\NodX}{\mathcal{N}_g(X,\beta)}
\newcommand{\NodGX}{\mathcal{N}^\Group_g(X,\beta)}
\newcommand{\NodGXpar}{{\mathcal{N}_g^{\Group}(X,\beta;\gamma)}}
\newcommand{\NodXpar}{\mathcal{N}_g(X,\beta;\gamma)}
\newcommand{\Divl}{\overline{\mathcal{D}}^{\Group}_{\{\m_1,...,\m_\ell\}}}
\newcommand{\Divisor}{\overline{\mathcal{D}}^{\Group}_{\m^0}}

